Challenges in Guardrailing Large Language Models for Science

The rapid development in large language models (LLMs) has transformed the landscape of natural language processing and understanding (NLP/NLU), offering significant benefits across various domains. However, when applied to scientific research, these powerful models exhibit critical failure modes related to scientific integrity and trustworthiness. Existing general-purpose LLM guardrails are insufficient to address these unique challenges in the scientific domain. We provide comprehensive guidelines for deploying LLM guardrails in the scientific domain. We identify specific challenges -- including time sensitivity, knowledge contextualization, conflict resolution, and intellectual property concerns -- and propose a guideline framework for the guardrails that can align with scientific needs. These guardrail dimensions include trustworthiness, ethics & bias, safety, and legal aspects. We also outline in detail the implementation strategies that employ white-box, black-box, and gray-box methodologies that can be enforced within scientific contexts.

==> chapter-2-notes.tex <==
\section{Literature Review Notes}

\subsection{Surveys}

\subsubsection{Safeguarding Large Language Models: A Survey}\cite{dong2024safeguarding}


\begin{itemize}
    \item techniques to evaluate, analyze, and \textcolor{red}{enhance some (un)desirable properties that a guardrail might want to enforce, such as hallucinations, fairness, privacy, and so on}.
    \item In societal contexts, \textcolor{red}{concerns also include the potential misuse by malicious actors through activities such as spreading misinformation or aiding criminal activities}.
    \item In the scientific context, LLMs can be used professionally, with dedicated ethical considerations and risks in scientific research.
    \item employing black-box, post-hoc strategies, notably guardrails, which monitor and filter the inputs and outputs of trained LLMs.
    \item \textcolor{red}{A guardrail is an algorithm that takes as input a set of objects (e.g., the input and the output of LLMs) and determines if and how some enforcement actions can be taken to reduce the risks embedded in the objects}.
    \item guardrails are used to identify the potential misuse in the query stage and to prevent the model from providing an answer that should not be given.
    \item \textcolor{red}{a guardrail of LLMs may include requirements from one or more categories: Hallucination, fairness, privacy, robustness, toxicity, legality, out-of-distribution, uncertainty, etc}.
    \item Llama Guard, Nvidia NeMo, and Guardrails AI.
    \item \textcolor{red}{Understand the existing guardrail frameworks that are being used to control model outputs in LLM services, as well as the techniques to evaluate, analyze, and enhance guardrails against specific desirable properties}.
    \item Understand the techniques that are being used to overcome these guardrails, as well as to defend the attacks and to reinforce the guardrails.
    \item \textcolor{red}{The primary performance review focuses on essential capabilities like language generation and complex reasoning}.
    \item \textcolor{red}{Safety analysis delves into the LLM’s alignment with human values, interactions with external environments, and integration into broader applications such as search engines}.
    \item Guardrails are applied during the interaction stage between users and deployed LLMs, the last step in the LLM lifecycle.
    \item Developers complete the development of guardrails through data processing, guardrail model training, and model customization or fine-tuning (e.g., Llama Guard and NeMo Guardrails).
    \item \textcolor{red}{The guardrails evaluate the output against the predefined rules to determine its compliance. If the content is deemed unsafe, guardrails may block it outright or issue a preset warning to the user}.
    \item Llama Guard.
    \item Llama Guard, developed by Meta on the Llama2-7b architecture, focuses on enhancing human-AI conversation safety. It is a fine-tuned model that takes the input and output of the victim model as input and predicts their classification on a set of user-specified categories.
    \item It lacks guaranteed reliability since the classification results depend on the LLM’s understanding of the categories and the model’s predictive accuracy.
    \item Nvidia Nemo.
    \item employs Colang, an executable program language, to establish constraints to guide LLMs within set dialogical boundaries.
    \item Nemo uses the "sentence-transformers/all-MiniLM-L6-v2" model to compute embeddings, which is used for the following KNN search (Annoy algorithm is employed for efficient nearest-neighbor search).
    \item \textcolor{red}{NeMo also includes a set of pre-implemented moderations dedicated to e.g., fact-checking, hallucination prevention in responses, and content moderation. NeMo is also a Type-1 neural-symbolic system, with its effectiveness closely tied to the performance of the KNN method}.
    \item Guardrails AI.
    \item Guardrails AI enables the user to add structure, type, and quality guarantees to the outputs of LLMs. It operates in three steps: 1) defining the “RAIL” spec, 2) initializing the “guard” and 3) wrapping the LLMs.
    \item the methods based on Guardrails AI are only applicable for text-level checks and cannot be used in multimodal scenarios involving images or audio.
    \item TruLens.
    \item TruLens, developed by TruEra1, is an open-source toolkit for developing, evaluating, and monitoring LLMs.
    \item Within TruLens, RAG’s role is to ensure the accuracy and relevance of model outputs by comparing them against predefined standards, thereby evaluating LLM apps.
    \item TruLens also visualizes the LLM applications’ rankings in a leaderboard according to their performance metrics, creating a dynamic environment that encourages developers to refine their models iteratively.
    \item TruLens is designed not to constrain LLM inputs and outputs but to provide a framework for continuous model refinement and evaluation, ensuring adherence to quality and relevance standards.
    \item Guidance AI.
    \item \textcolor{red}{Guidance AI2, a programming paradigm, offers superior control and efficiency than conventional prompting and chaining. It allows users to constrain generation (e.g., with regex and CFGs) and interleave control (conditional, loops) and generation seamlessly}.
    \item At any timestep during the program execution, the language model can be called for generation (via \{\{gen\}\} tag) or to make logical flow decisions, such as \{\{\#select\}\}\{\{or\}\}\{\{/select\}\} commands.
    \item using token healing to optimize prompt boundaries.
    \item Regex patterns to enforce formatting.
    \item Guidance’s templated output is more suitable for generating text with high formatting requirements, such as ensuring legally compliant and controllable JSON structures.
    \item During this process, different operation commands have their processing methods; for example, encountering the select command, it specifies the generation of a token and returns the corresponding log probs, then uses a trie tree to match candidates and determine their probabilities, finally selecting the one with the highest probability.
    \item LMQL (Language Model Query Language).
    \item LMQL 3, a programming interface for LLMs focusing on controlled output and safety of generated content.
    \item Building on the foundation of Guidance AI, the LMQL project further advances the concept of “prompt templates” into a new programming language paradigm. As a Python superset, it allows developers the capacity to embed precise constraints within their queries.
    \item constraints, from content restriction to adherence to specific formats for accuracy, leverage logit masking and custom operator support for fine-tuned control.
    \item At its core, LMQL’s runtime and decoding ability uniquely features employs a scripted Beam search to execute LMQL-specific queries and constraints.
    \item Follow[<expr>]pu,tq is designed to guide the generation process by evaluating the impact of adding a new token t to the current interaction trace u on meeting the specified constraints.
    \item Python Packages.
    \item LangChain: LangChain is pivotal in streamlining the development of LLM applications. It introduces components that can be leveraged to implement guardrails, thus indirectly contributing to creating safer and more reliable AI solutions.
    \item AI Fairness 360 (AIF360): AIF360 is an extended toolkit from IBM that provides developers with a comprehensive set of algorithms designed to detect, understand and mitigate bias in AI models.
    \item Adversarial Robustness Toolbox (ART): ART is tailored to enhance model security and robustness in the face of increasing adversarial attacks.
    \item Fairlearn: This package addresses and reduces unwanted biases in machine learning models. Fairlearn provides developers with tools and methodologies to assess and mitigate biases, fostering fairness and equality in AI outcomes.
    \item Detoxify: Detoxify aims to identify and mitigate toxic content in text data, serving as a crucial tool for maintaining a respectful and safe digital interaction space.
    \item we focus on hallucination, fairness, privacy, robustness, toxicity, legality, out-of-distribution, and uncertainty.
    \item Hallucination.
    \item Hallucinations in LLMs are defined as responses that are either nonexistent in reality, illogical, or irrelevant to the prompt provided.
    \item In certain contexts, such as safety-critical applications, ensuring rigorous guarantees for the output of LLMs is imperative and achievable. This involves first specifying high-level formal specifications and then applying formal verifiers to monitor whether the execution of LLMs conforms to the specified requirements.
    \item authors proposed a framework for counterexample-guided inductive synthesis using LLMs and satisfiability modulo theory (SMT). Within this framework, an SMT solver is employed to eliminate the hallucinated outputs of the LLM, guiding it to generate correct outputs.
    \item utilizing continuous integration (CI) to automatically identify hallucinations in the outputs of an LLM with the aid of another LLM. The CI process involves regular incremental updates to the software, with each change automatically built and tested, allowing for prompt detection of errors.
    \item Instead of using another LLM to identify the errors, some researchers use trusted information sources to cross-check the generated content.
    \item Different methodologies have been adopted for output evaluation, such as binary judgment mechanisms and using a k-point Likert scale.
    \item Fairness.
    \item Fairness is a concept that originates in sociology, economics, and law. It is defined as “imperfect and just treatment or behavior without favoritism or discrimination” in the Oxford English Dictionary.
    \item The key to fairness in NLP is the presence of social biases in language models.
    \item Fairness in LLMs has been studied from different angles, such as gender bias, cultural bias, dataset bias, and social bias.
    \item Biases are purposefully introduced into the responses of LLMs to craft distinct personas for use in interactive media.
    \item DAMA utilizes causal analysis to identify problematic model components, mainly focusing on mid-upper feedforward layers most prone to convey biases.
    \item a Bias Index is designed to quantify and address biases inherent in LLMs, including GPT-4.
    \item A Counterfactual Data Augmentation (CDA) is a widespread data processing method to balance labels, which replaces the sensitive attributes in the original sample with the sensitive attributes of the opposite demographic based on a prior list of sensitive word pairs.
    \item For instance, FairBERTa is a fairer model for retraining RoBERTa on a large-scale demographic perturbation corpus Perturbation Augmentation NLP Dataset (PANDA) containing 98K augmentation sample pairs.
    \item Moreover, an additional debiasing module is added after the encoder of LLMs to filter out the bias in the representation, and a common strategy is to utilize a contrastive learning framework for training.
    \item Many studies have concentrated on reducing bias through model adaptation approaches.
    \item bias depends not solely on the number of parameters but also on factors like perplexity and that techniques like debiasing of OPT using LoRA can significantly reduce bias.
    \item Instead of fine-tuning parameters, several studies directly set up guardrails on the interaction between users and LLMs by exploring the control of input and output.
    \item using purposely designed code generation templates to mitigate the bias in code generation tasks.
    \item cultural prompting is a simple and effective method to reduce cultural bias in the latest LLMs.
    \item Developing guardrails through a comprehensive approach that intertwines various strategies is crucial to mitigate bias effectively.
    \item Privacy (Copyright).
    \item the need for cautious and robust data handling protocols.
    \item Differential Privacy (DP)-tuned LLMs emerge as a leading approach to protecting data privacy in these contexts, ensuring secure handling of sensitive information by LLMs.
    \item For general NLP models, indicated that a direct application of DP-SGD may not perform satisfactorily.
    \item Privacy Protection Language Models (PPLM), a novel paradigm for fine-tuning LLMs that incorporates domain-specific knowledge while preserving data privacy.
    \item a “Just Fine-tune Twice" (JFT) framework for the latest large Transformer models, achieving Selective Differential Privacy protection.
    \item Other than constructing privacy-preserving LLMs, watermarking techniques can play a more critical role in LLMs for privacy and copyright protection.
    \item A typical watermarking mechanism embedded watermarks into the output of LLMs by selecting a randomized set of “green” tokens before a word is generated and then softly promoting the use of green tokens during sampling.
    \item LLMs also risk user trust due to their pre-training on vast textual datasets, potentially leading to inadvertent disclosure of sensitive information about individuals.
    \item In addressing privacy concerns within LLM applications, implementing guardrails is crucial for existing and in-development technologies.
    \item Implementing content control mechanisms such as blocklists, allowlists, and suppression lists directly tackles unsafe content generation that could compromise privacy.
    \item Regular model retraining to align with current norms and the option to revert to previous safe versions of the model serve as dynamic responses to privacy challenges.
    \item Implementing selective memory and information filtering techniques restricts the AI’s access to sensitive data, directly safeguarding user privacy.
    \item Removing personally identifiable information (PII) from data used in model training is critical in protecting privacy.
    \item Robustness.
    \item \textcolor{red}{With the rise of LLMs as dominant models in NLP, robustness consists of out-of-distribution (OOD) and adversarial robustness}.
    \item The adversary (end-user) only attempts to jailbreak the model by explicitly optimizing adversarial queries or adaptively making queries based on previous outputs but will not make out-of-distribution queries asking about potentially revoked information.
    \item \textcolor{red}{Let $x$ represent the input and $y$ its corresponding correct label. Consider a model $f$ that has been trained on data pairs $(x, y) \in D$, with its output prediction for $x$ given by $f(x)$. When new test data $(x_1, y_1) \in D_1$, where $D_1$ is not identical to $D$, is introduced, the robustness of the model can be determined by its performance on $D_1$ through comprehensively perturbing the input from $x$ to $x_1$}.
    \item \textcolor{red}{The adversarial robustness under the LLMs refers to the ability of models to maintain performance when faced with inputs that have been intentionally altered or crafted to cause the model to error, such as the malicious queries made intentionally or unintentionally}.
    \item In particular, disturbances are directed at various layers of linguistic signals, including characters, words, sentence structures, and underlying meanings. The core objective is to replicate potential user mistakes (e.g. use of near-meaning words), to assess the impact of minor deviations on the outcomes of LLMs.
    \item Typically, guardrails pre-process users’ inputs to remove or neutralize potentially adversarial content, thus preventing models from being misled by manipulated inputs (e.g., correcting typos and standardizing input formats).
    \item guardrails also monitor LLM’s outputs.
    \item Toxicity.
    \item \textcolor{red}{LLMs, as one of the prevalent developments in traditional language modeling, are frequently trained using vast quantities of datasets, which can include content exhibiting toxic behavior and unsafe material, such as hate speech, offensive/abusive language, etc}.
    \item The definition of what constitutes toxicity of the LLMs varies normally, toxicity responses will be defined as rude, disrespectful, or unreasonable responses that are likely to make an individual leave a discussion.
    \item Existing studies address the problem by focusing on representative terms in datasets, such as identity terms.
    \item studies leveraged standard toxicity metrics, such as the Toxicity Classifier Score and PerspectiveAPI, to determine whether the LLM’s response is toxic.
    \item typical metrics are susceptible to evaluator bias, and encoders are perturbed.
    \item Even when a generative model is trained on data characterized by low toxicity levels, and its ability to minimize the generation of toxic text has been validated through evaluations, it is still crucial to enforce protective measures during live interactions between users and the model.
    \item Legality.
    \item managing the risks associated with illicit outputs.
    \item safeguarding efforts on two fronts: implementing measures to reject inappropriate user inputs and moderating model output to ensure it is appropriate and safe for users or downstream tasks.
    \item measures include: i) researchers meticulously screen and clean the training data before training the models to remove inappropriate, harmful, or illegal content.
    \item During model training, human reviewers assess the samples generated by the model and offer feedback, aiding in rectifying errors and enhancing the model’s output.
    \item Once the model construction is completed and before release, models undergo thorough and rigorous ethics and safety testing.
    \item One classical approach is red teaming.
    \item Organizations like OpenAI, Anthropic, Google, and Meta utilize diverse methodologies for red teaming, ensuring a thorough evaluation and effective risk mitigation.
    \item monitoring systems are established upon model release to detect inappropriate inputs and outputs.
    \item Upon identification of any issues, immediate measures, such as content filtering algorithms or human intervention protocols, are swiftly implemented to address the concern.
    \item One notable application of LangChain in the legal domains is ConstitutionalChain. By incorporating predefined rules and guidelines, ConstitutionalChain can filter and modify generated content to align with constitutional principles.
    \item Out-of-Distribution.
    \item out-of-distribution (OOD) data strictly refers to data not belonging to any in-distribution classes used in training.
    \item due to the immense training corpora used for LLMs, making it difficult to define precisely what data has not been utilized for training.
    \item the generative nature of LLMs adds another layer of complexity to defining the OOD problem.
    \item To mitigate the impact of OOD on model performance in practical tasks, strategies such as setting up anomaly input filtering mechanisms or constructing OOD detectors tailored to the task can be employed.
    \item Uncertainty.
    \item A key aspect of LLMs’ trustworthiness lies in their ability to discern their outputs’ reliability and correctness, a concept central to uncertainty quantification.
    \item The effectiveness of uncertainty quantification is further contingent on the alignment between the model’s predicted confidence and its actual accuracy, essentially measuring the model’s calibration.
    \item the calibration of LLMs is improved relatively through techniques like combining multiple reasoning chains, integrating different prompts, or by prompting LLMs to output their confidence levels directly.
    \item \textcolor{red}{KnowNo, a framework designed to measure and align the uncertainty in LLM-based planners, enabling them to recognize their limitations and seek assistance when necessary}.
    \item The primary hurdles in assessing LLM uncertainty arise from the pivotal roles of meaning and structure in language.
    \item concept of semantic entropy, which integrates linguistic consistencies arising from identical meanings.
    \item \textcolor{red}{The fundamental method involves a semantic equivalence relation, denoted as $\epsilon(s_i, s_j)$, where $s_i$ and $s_j$ represent output sentences corresponding to a given input. This equivalence relation is said to hold when two sentences $s_i$ and $s_j$ convey the same meaning, implying that they belong to the same cluster $C$. The semantic entropy is defined as $H(C|x) = - \sum_{C} P(C|x) \ln P(C|x)$}.
    \item In a white-box scenario, the attacker has full visibility into the model’s parameters.
    \item A black-box situation restricts the attacker from observing the model’s outputs.
    \item In a grey-box context, the attacker has partial access, typically to some training data.
    \item White-box Jailbreaks.
    \item A white-box attack normally refers to a scenario in which the attacker has full access to the internal details of the model.
    \item Learning-based Methods.
    \item The Greedy Coordinate Gradient (GCG) method was designed to search a specific sequence of characters (an adversarial suffix). When the adversarial suffix is attached to different queries, it misleads the LLM to generate a response with harmful content.
    \item COLDAttack adopts a new jailbreak, to automate the search of adversarial LLM attacks under a variety of restrictions such as fluency, stealthiness, sentiment, and left-right-coherence. It performs efficient gradient-based sampling in the continuous logit space and relies on a guided decoding process to translate the continuous logit sequences back into discrete text.
    \item LLM Generation Manipulation.
    \item Black-box Jailbreaks.
    \item black-box attacks operate under the premise that adversaries lack knowledge of the LLM’s internal architecture or parameters.
    \item jailbreak attacks conducted within a black-box setting are classified into four categories: i) manually designed jailbreaks, ii) attacks exploiting long-tail distribution, iii) optimization-based methods for generating jailbreaks, and iv) unified framework for jailbreaking.
    \item A prompt-based jailbreak method, called DeepInception, was devised for conducting a black-box attack on LLMs. This involves injecting an inception mechanism into an LLM and effectively hypnotizing it to act as a jailbreaker. DeepInception explicitly constructs a nested scene to serve as the inception for guiding the behavior of the LLM. This nested scene facilitates an adaptive approach to circumvent safety constraints in a normal scenario, opening up the potential for subsequent jailbreaks.
    \item In-Context Attack (ICA). ICA is tailored to construct malicious contexts to direct models to produce harmful outputs. The efficacy of in-context demonstrations in aligning LLMs is demonstrated, and implementing these methods is straightforward.
    \item Exploiting Long-tail Distribution.
    \item CipherChat is designed with three key elements in its system prompt to ensure effective communication through ciphers: (1) behavior assignment, (2) cipher teaching, and (3) enciphered unsafe demonstrations. It enables users to interact with LLMs using cipher prompts, system role descriptions, and few-shot enciphered demonstrations.
    \item Prompt Injection for Desired Responses.
    \item LoFT (Local Proxy Fine-tuning) to fine-tuning smaller, local proxy models to develop attacks that are more likely to transfer successfully to larger, more complex LLMs. This technique leverages the target LLMs to produce prompts closely aligned with harmful queries, effectively gathering prompts from a localized vicinity around these queries.
    \item Techniques for Strengthening LLMs.
    \item Detection-based Methods: Guardrail Enhancement.
    \item To detect the harmful information in the user’s input, PPL calculates the perplexity of a provided input to decide whether a user’s request should be accepted or rejected.
    \item SmoothLLM borrowed the idea of randomized smoothing literature, it randomly alters multiple versions of a given input and then combines the respective predictions to identify adversarial inputs.
    \item In-Context Defense (ICD) method is designed to bolster model resilience by demonstrations of rejecting to answer harmful prompts via in-context demonstration.
    \item To defend LLM attacks, LLM SELF DEFENSE was proposed first. Specifically, by incorporating the generated content into a pre-defined prompt and using another instance, LLM, to analyze the text, it constructs an extra guardrail filter for preventing harmful content.
    \item a moving target defense (MTD) to enhance the LLM system. Compared to previous guardrail methods that decide whether the input/output is safe, MTD calculates a composite score for each response by combining its quality and toxicity metrics. It employs randomization to select a response that qualifies both response metrics, eventually providing a solid moving target defense for the LLMs.
    \item Mitigation-based Methods: Affirmative Response Generation.
    \item novel inference method, Rewindable Autoregressive INference (RAIN) enables pre-trained LLMs to assess their own outputs and leverage the assessment outcomes to inform and steer the backtracking and generating content to enhance AI safety.
    \item Self-Reminder suggests that adding self-reminder prompts can be an effective defense. They speculate that initiating ChatGPT with a ‘system mode’ prompt at the most external level to remind it of its role as a responsible AI tool could reduce its vulnerability to being malevolently steered by user inputs at a deeper level.
    \item concatenating an extra system prompt after the user’s query that reminds the LLMs to respond responsibly, the experimental results showed that self-reminders significantly reduce the success rate of jailbreak attacks.
    \item a multi-round automatic red-teaming framework MART to improve the scalability of safety alignment. Two players, i.e., an adversarial LLM and a target LLM, iteratively interplay with each other. The adversarial LLM aims to generate challenging prompts that provoke unsafe responses from the target LLM.
    \item SafeDecoding found that despite the likelihood of tokens signifying harmful content being higher than those for harmless responses, safety disclaimers continue to emerge among the highest-ranking tokens when sorted by probability in descending order.
    \item in the training phase, the model will be fine-tuned with a few safety measures, and then, during the inference, SafeDecoding further constructs the new token distribution.
    \item Conflicting Requirements.
    \item Conflicting requirements are typical, including, e.g., fairness and privacy, privacy and robustness, and robustness and fairness.
    \item Integrating guardrails with LLMs may lead to a discernible conservative shift in the generation of responses to open-ended text-generation questions.
    \item How can exploratory depth be maintained in responses, particularly for open-ended test generation tasks?
    \item Furthermore, does the application of guardrails constrain ChatGPT’s capacity to deliver more intuitive responses?
    \item adoption of guardrails has also led to the model adopting a more concise communication approach, offering fewer details and electing non-response in specific queries.
    \item The decision “to do or not to do” can be challenging when designing the guardrail. While the most straightforward approach is to decline an answer to any sensitive questions, is it the most intelligent one? That is, we need to determine if the application of guardrail always has a positive impact on LLMs that is within our expectation.
    \item Prior research suggested incorporating a creativity assessment mechanism into the guardrail development for LLMs.
    \item Multidisciplinary Approach.
    \item It is reasonable to expect future guardrails to integrate harm detections and other mechanisms to deal with, e.g., ethics, fairness, and creativity.
    \item In domain-specific scenarios, specialized rules may conflict with the general principles.
    \item the concrete requirements for guardrails will differ across different LLMs, and research is needed to scientifically determine requirements.
    \item Developing LLMs ethically involves adhering to fairness, accountability, and transparency. These principles ensure that LLMs do not perpetuate biases or cause unintended harm.
    \item the ethical development of LLMs is not a one-time effort but requires ongoing evaluation and refinement. These tasks involve regular assessment of LLMs outputs, updating models to reflect changing societal norms, and incorporating feedback from diverse user groups to ensure that LLMs remain fair and unbiased.
    \item To manage the complexity, the whole system approach, which promotes an ongoing and dynamic way of working and enables local stakeholders to come together for an integrated solution, has been successfully working on healthcare systems.
    \item a guardrail requires the cooperation of symbolic and learning-based methods. For example, we may expect that the learning agents deal with the frequently-seen cases (where there are plenty of data) to improve the overall performance w.r.t. the requirements mentioned above, and the symbolic agents take care of the rare cases (where there are few or no data) to improve the performance in dealing with corner cases in an interpretable way.
    \item Systems Development Life Cycle (SDLC) The criticality of guardrails requires a careful engineering process.
    \item Rigorous verification and testing will be needed, which requires a comprehensive set of evaluation methods.
    \item The Pareto front is a concept from the field of multi-objective optimization. It represents a set of non-dominated solutions, where no other solutions in the solution space are better when all objectives are considered.
    \item attention should also be paid to understanding the theoretical limits of the evaluation methods, e.g., randomized smoothing causes a fairness problem.
    \item Safeguards for LLM Agents.
    \item These LLM agents typically encompass five fundamental modules: LLMs, planning, action, external tools, and memory and knowledge.
    \item increased autonomy raises concerns about unintended consequences, especially in sensitive domains like scientific research.
    \item Due to their autonomy, LLM agents introduce higher complexity and unpredictability. The integration of decision-making processes means they might initiate actions that are hard to foresee or control, potentially leading to ethical and practical risks.
    \item For LLM agents, “safeguard" means implementing stricter controls and oversight to manage their broader capabilities effectively.
    \item In summary, Guardrails are highly complex due to their role in managing interactions between LLMs and humans. A systematic approach, supported by a multidisciplinary team, can fully consider and manage the complexity and provide assurance to the final product.
\end{itemize}

\begin{table}[h]
    \centering
    \caption{Abilities among different Guardrails, Dong \textit{et al.}}  \begin{tabular}{lcccccc}
        \hline
        & Llama Guard & Nvidia NeMo Guardrails & AI TruLens & Guidance AI & LMQL \\
        \hline
        Hallucination & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
        Fairness & \checkmark & - & \checkmark & \checkmark & - & - \\
        Privacy & - & \checkmark & - & - & - & - \\
        Robustness & - & - & - & - & - & - \\
        Toxicity & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
        Legality & \checkmark & - & - & - & - & - \\
        Out-of-Distribution & - & - & \checkmark & - & - & - \\
        Uncertainty & - & \checkmark & \checkmark & \checkmark & - & - \\
        \hline
    \end{tabular}
\end{table}

\begin{table}[H]
    \centering
    \caption{Comparison among Different Jailbreaks for (Guarded) LLMs, Dong \textit{et al.}}
    \begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|p{3.5cm}|p{1.5cm}|p{2cm}|p{3cm}|}
        \hline
        \textbf{Attack} & \textbf{Access Type} & \textbf{Prompt Level} & \textbf{Core Technique} & \textbf{Stealthiness} & \textbf{GPT4 Evaluation} & \textbf{Targeted Property} \\
        \hline
        GCG [65] & White & User & Greedy Gradient-based Search & Low & $\hat{}$ & Harmful Content \\
        PGD [126] & White & User & Continuous Relaxation \& Entropy projection & Low & $\hat{}$ & Harmful Content \\
        PRP* [127] & White & User & In-context Learning \& two-step prefix-based & Low & $\hat{}$ & Harmful Content \\
        AutoDAN-Liu* [128] & White & System+User & Hierarchical Genetic Algorithm & High & \checkmark & Harmful Content \\
        AutoDAN-Zhu* [129] & White & User & Double-loop Optimization & High & \checkmark & Harmful Content \& prompt leaking \\
        COLD-Attack* [130] & White & User & Langevin dynamics & High & $\hat{}$ & Harmful Content \\
        ProMan [131] & White & - & Generation Manipulation & - & $\hat{}$ & Harmful Content \& Privacy Leakage \\
        JailBroken [132] & Black & System & Failure modes as guiding principles & Low & \checkmark & Harmful Content \& personally identifiable information leakage \\
        DeepInception [133] & Black & User & Nested instruction & Medium & \checkmark & Harmful Content \\
        DAN* [125] & Black & User & Characterizing in-the-wild prompt & High & \checkmark & Harmful Content \\
        ICA [134] & Black & User & In-context learning ability of LLM & Low & $\hat{}$ & Harmful Content \\
        SAP [135] & Black & User & In-context learning ability of LLM & Medium & $\hat{}$ & Harmful Content \\
        DRA [136] & Black & User & Making Them Ask and Answer & Low & \checkmark & Harmful Content \\
        CipherChat [137] & Black & System & Long-tail: cipher & High & \checkmark & Harmful Content \\
        MultiLingual [138] & Black & User & Long-tail: low-resource & High & \checkmark & Harmful Content \\
        LRL [139] & Black & User & Long-tail: low-resource & High & \checkmark & Harmful content \\
        CodeChameleon [140] & Black & User & Long-tail: encrypts & High & \checkmark & Harmful Content \\
        ReNeLLM [141] & Black & User & Prompt rewriting \& scenario nesting & High & \checkmark & Harmful Content \\
        PAIR [142] & Black & System & Automatic Iterative Refinement & High & \checkmark & Harmful content \\
        GPTFUZZER [143] & Black & User & Fuzzing & Low & \checkmark & Harmful content \\
        TAP [144] & Black & System & Tree-of-thought reasoning & Medium & \checkmark & Harmful content \\
        Mosaic Prompts [145] & Black & User & Semantic censorship & High & $\hat{}$ & Impermissible content \\
        EasyJailbreak [146] & Black & System+User & Unified framework for 12 jailbreaks & - & \checkmark & Jailbreak attack evaluation \\
        PROMPTINJECT [147] & Black & User & Mask-based iterative strategy & Low & $\hat{}$ & Goal hijacking \& prompt leaking \\
        IPI [148] & Black & System & Indirect prompt injection & High & \checkmark & Cyber threats like theft of data and denial of service etc. \\
        HOUYI [149] & Black & User & SQL injection \& XSS attacks & Low & $\hat{}$ & Prompt abuse \& prompt leak \\
        GA [150] & Black & User & Genetic algorithm & Low & $\hat{}$ & Harmful content \\
        GUARD [151] & Black & System+User & Role-playing LLMs & High & $\hat{}$ & Harmful content \\
        CIA [152] & Black & User & Combination of multiple instructions & Medium & \checkmark & Harmful content \\
        Pelrine et al. [153] & Grey & User & Fine-tuning & Low & \checkmark & Misinformation \& Privacy Leakage \\
        Zhang et al. [154] & Grey & User & Fine-tuning & Low & \checkmark & Harmful content \\
        Safety-tuned [155] & Grey & User & Fine-tuning & Low & $\hat{}$ & Harmful content \\
        Janus inference [156] & Grey & System & Fine-tuning & Low & $\hat{}$ & Privacy Leakage \\
        Qi et al. [157] & Grey & User & Fine-tuning & Low & $\hat{}$ & Harmful content \\
        Pelrine et al. [153] & Grey & User & Poisoning knowledge retrieval & Medium & \checkmark & Harmful content \& fairness \\
        PoisonedRAG [158] & Grey & System & Poisoning knowledge retrieval & Low & \checkmark & Hallucination \\
        AutoPoison [159] & Grey & System & Content Injection & Low & $\hat{}$ & Triggered response \\
        LoFT [160] & Grey & System & Fine-tuning & Low & \checkmark & Harmful content \\
        BadGPT [161] & Grey & System & Backdoor Attack & Medium & $\hat{}$ & Harmful content \\
        ICLAttack [162] & Grey & System & Backdoor Attack & Low & $\hat{}$ & Triggered response \\
        ActivationAttack [163] & Grey & System & Activation Steering & Low & $\hat{}$ & Harmful \& Biased content \\
        \hline
    \end{tabular}
\end{table}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/dong2024-1.png}
    \caption{Guardrails Lifecycle and Vulnerabilities}
    \label{fig:dong2024-1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/dong2024-2-llamaguard.png}
    \caption{\textit{Llama Guard} Guardrail Workflow}
    \label{fig:dong2024-2}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/dong2024-3-nvidia-nemo.png}
    \caption{\textit{Nvidia NeMo} Guardrail Workflow}
    \label{fig:dong2024-3}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/dong2024-4-guardrailsai.png}
    \caption{\textit{Guardrails AI} Workflow}
    \label{fig:dong2024-4}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/dong2024-5-trulens.png}
    \caption{\textit{Truelens} Workflow}
    \label{fig:dong2024-5}
\end{figure}


\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/dong2024-6-guidance.png}
    \caption{\textit{Guidance AI} Workflow}
    \label{fig:dong2024-6}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/dong2024-7-lmql.png}
    \caption{\textit{LMQL} Workflow}
    \label{fig:dong2024-7}
\end{figure}


\subsubsection{Building Guardrails for Large Language Models}\cite{dong2024building}


Annotations

\hfill

\iffalse
\begin{itemize}
    \item \textcolor{red}{Guardrails, which filter the inputs or outputs of LLMs, have emerged as a core safeguarding technology}.
    \item \textcolor{red}{the rapid deployment and integration of LLMs have raised significant concerns regarding their risks including, but not limited to, ethical use, data biases, privacy and robustness}.
    \item The difficulty in constructing guardrails often lies in establishing the requirements for them.
    \item \textcolor{red}{a guardrail of LLMs may include requirements from one or more of the following categories: (i) Free from unintended responses e.g., offensive and hate speech; (ii) Compliance to ethical principles such as fairness, privacy, and copyright; (iii) Hallucinations and uncertainty}.
    \item \textcolor{red}{The need to work with multiple requirements makes it worse, especially when some requirements can be conflicting}.
    \item For vulnerability detection, the victim LLMs are typically treated as a blackbox, and thus they can be either with or without guardrails.
    \item Protection via LLMs enhancement includes techniques that tune the weights of LLMs.
    \item For protection via I/O engineering, we consider any techniques that work on input and output, e.g., prompt engineering and output filter.
    \item Most research uses prompt engineering methods to cause LLMs to create unintended content, a process often referred to as “jailbreaking”.
    \item Vulnerability Detection.
    \item \textcolor{red}{LLMs can be manipulated to produce malicious contents using specific prompts}.
    \item automated prompt generation based on gradient.
    \item Protection via LLMs Enhancement The LLMs can be enhanced by inherent safety training technologies.
    \item \textcolor{red}{incorporate a safety reward into the RLHF process to prevent harmful outputs}.
    \item implementing context distillation in the training dataset.
    \item The robustness of language models can also be improved by modifying the training loss functions.
    \item ineffective for the LLMs due to the catastrophic forgetting in the training process.
    \item approaches require retraining of the LLMs to defend against the attacks, which can be unsuitable due to high-cost and closed-source nature.
    \item Protection via I/O Engineering.
    \item several I/O engineering approaches that work on the input/output prompts have emerged.
    \item defense technologies, including preprocessing and rephrasing input prompts.
    \item randomized smoothing technology to defend against such attacks by modifying input prompts and using majority voting for detection.
    \item \textcolor{red}{the defenses are effective against certain attacks, they remain vulnerable to stronger ones. This could turn into a continuous and infinite cycle of attacks and defenses}.
    \item \textcolor{red}{it is necessary to develop metrics for toxicity and other criteria to address unintended responses}.
    \item we can consider certified robustness bounds, either statistical bound or deterministic bound, as scores to measure the guardrail performance.
    \item Limisiewicz et al. (2023) provided a bias mitigating method, DAMA, that can reduce bias while maintaining model performance on downstream tasks.
    \item bias is not solely dependent on the number of parameters but also on factors like perplexity, and that techniques like debiasing of OPT using LoRA can significantly reduce bias.
    \item Protection via I/O Engineering.
    \item cultural prompting is a simple and effective method to reduce cultural bias in the latest LLMs, although it may be ineffective or even exacerbate bias in some countries.
    \item Hallucinations and Uncertainty.
    \item \textcolor{red}{The hallucinations in conditional text generation are closely tied to high model uncertainty}.
    \item The absence of uncertainty measures for LLMs significantly hampers the reliability of information generated by LLMs.
    \item Manakul et al. (2023) proposed to identify hallucinations by generating multiple responses and evaluating the consistency of factual statements.
    \item mitigating data-related hallucinations in LLMs by increasing the amount of factual data during the pretraining phase.
    \item Modifying the training dataset can partially reduce the model’s knowledge gap effectively.
    \item Liang et al. (2024) developed an automated hallucination annotation tool, DreamCatcher, and proposing a Reinforcement Learning from Knowledge Feedback training framework, effectively improving their performance in tasks related to factuality and honesty.
    \item recommend using retrieval-augmented methods, which seek to add external knowledge acquired from retrieval directly to the LLMs’ prompt.
    \item Dhuliawala et al. (2023) introduced the “Chain-of-Verification” method to effectively reduce the generation of inaccurate information in LLMs.
    \item Zhao et al. (2023) proposed a Verify-andEdit framework based on GPT-3, which enhances the factual accuracy of predictions in open-domain question-answering tasks.
    \item Gao et al. (2023) pioneered the “Retrofit Attribution using Research and Revision” system, which improves the outputs by automatically attributing and postediting generated text to correct inaccuracies.
    \item Kuhn et al. (2022) presented the concept of semantic entropy, an entropy that integrates linguistic invariances brought about by the same meaning.
    \item Challenges on Designing Guardrails.
    \item \textcolor{red}{Conflicting requirements are typical, including e.g., fairness and privacy, privacy and robustness, and robustness and fairness}.
    \item \textcolor{red}{Although capabilities typically remain constant, behavior can alter due to fine-tuning, which can be interpreted as the “uncertainty” challenges in LLMs}.
    \item \textcolor{red}{The decision of “to do or not to do” can be a challenging task when designing the guardrail}.
    \item a guardrail requires the cooperation of symbolic and learning-based methods.
\end{itemize}
\fi

\begin{itemize}
    \item \textbf{Guardrails Properties}
    \begin{itemize}
        \item \textcolor{red}{Guardrails, which filter the inputs or outputs of LLMs, have emerged as a core safeguarding technology}.
        \item \textcolor{red}{a guardrail of LLMs may include requirements from one or more of the following categories: (i) Free from unintended responses e.g., offensive and hate speech; (ii) Compliance to ethical principles such as fairness, privacy, and copyright; (iii) Hallucinations and uncertainty}.
        \item The difficulty in constructing guardrails often lies in establishing the requirements for them.
        \item \textcolor{red}{The need to work with multiple requirements makes it worse, especially when some requirements can be conflicting}.
        \item a guardrail requires the cooperation of symbolic and learning-based methods.
        \item The decision of “to do or not to do” can be a challenging task when designing the guardrail.
        \item \textcolor{red}{Conflicting requirements are typical, including e.g., fairness and privacy, privacy and robustness, and robustness and fairness}.
    \end{itemize}

    \item \textbf{Ethical and Privacy Concerns}
    \begin{itemize}
        \item \textcolor{red}{the rapid deployment and integration of LLMs have raised significant concerns regarding their risks including, but not limited to, ethical use, data biases, privacy and robustness}.
        \item For vulnerability detection, the victim LLMs are typically treated as a blackbox, and thus they can be either with or without guardrails.
    \end{itemize}

    \item \textbf{Vulnerability Detection}
    \begin{itemize}
        \item Vulnerability Detection.
        \item \textcolor{red}{LLMs can be manipulated to produce malicious contents using specific prompts}.
        \item Most research uses prompt engineering methods to cause LLMs to create unintended content, a process often referred to as “jailbreaking”.
        \item automated prompt generation based on gradient.
    \end{itemize}

    \item \textbf{LLM Enhancement and Protection}
    \begin{itemize}
        \item Protection via LLMs Enhancement The LLMs can be enhanced by inherent safety training technologies.
        \item \textcolor{red}{incorporate a safety reward into the RLHF process to prevent harmful outputs}.
        \item implementing context distillation in the training dataset.
        \item The robustness of language models can also be improved by modifying the training loss functions.
        \item ineffective for the LLMs due to the catastrophic forgetting in the training process.
        \item approaches require retraining of the LLMs to defend against the attacks, which can be unsuitable due to high-cost and closed-source nature.
    \end{itemize}

    \item \textbf{I/O Engineering for Protection}
    \begin{itemize}
        \item Protection via I/O Engineering.
        \item For protection via I/O engineering, we consider any techniques that work on input and output, e.g., prompt engineering and output filter.
        \item several I/O engineering approaches that work on the input/output prompts have emerged.
        \item defense technologies, including preprocessing and rephrasing input prompts.
        \item randomized smoothing technology to defend against such attacks by modifying input prompts and using majority voting for detection.
        \item \textcolor{red}{the defenses are effective against certain attacks, they remain vulnerable to stronger ones. This could turn into a continuous and infinite cycle of attacks and defenses}.
    \end{itemize}

    \item \textbf{Bias Mitigation}
    \begin{itemize}
        \item Limisiewicz et al. (2023) provided a bias mitigating method, DAMA, that can reduce bias while maintaining model performance on downstream tasks.
        \item bias is not solely dependent on the number of parameters but also on factors like perplexity, and that techniques like debiasing of OPT using LoRA can significantly reduce bias.
        \item Protection via I/O Engineering.
        \item cultural prompting is a simple and effective method to reduce cultural bias in the latest LLMs, although it may be ineffective or even exacerbate bias in some countries.
    \end{itemize}

    \item \textbf{Hallucinations and Uncertainty}
    \begin{itemize}
        \item Hallucinations and Uncertainty.
        \item \textcolor{red}{The hallucinations in conditional text generation are closely tied to high model uncertainty}.
        \item The absence of uncertainty measures for LLMs significantly hampers the reliability of information generated by LLMs.
        \item Manakul et al. (2023) proposed to identify hallucinations by generating multiple responses and evaluating the consistency of factual statements.
        \item mitigating data-related hallucinations in LLMs by increasing the amount of factual data during the pretraining phase.
        \item Modifying the training dataset can partially reduce the model’s knowledge gap effectively.
        \item Liang et al. (2024) developed an automated hallucination annotation tool, DreamCatcher, and proposing a Reinforcement Learning from Knowledge Feedback training framework, effectively improving their performance in tasks related to factuality and honesty.
        \item recommend using retrieval-augmented methods, which seek to add external knowledge acquired from retrieval directly to the LLMs’ prompt.
        \item Dhuliawala et al. (2023) introduced the “Chain-of-Verification” method to effectively reduce the generation of inaccurate information in LLMs.
        \item Zhao et al. (2023) proposed a Verify-andEdit framework based on GPT-3, which enhances the factual accuracy of predictions in open-domain question-answering tasks.
        \item Gao et al. (2023) pioneered the “Retrofit Attribution using Research and Revision” system, which improves the outputs by automatically attributing and postediting generated text to correct inaccuracies.
        \item Kuhn et al. (2022) presented the concept of semantic entropy, an entropy that integrates linguistic invariances brought about by the same meaning.
    \end{itemize}

    \item \textbf{Guardrail Design Challenges}
    \begin{itemize}
        \item Challenges on Designing Guardrails.
        \item \textcolor{red}{Although capabilities typically remain constant, behavior can alter due to fine-tuning, which can be interpreted as the “uncertainty” challenges in LLMs}.
    \end{itemize}
\end{itemize}

\hfill

\subsubsection{Verify-and-Edit: A Knowledge-Enhanced Chain-of-Thought Framework}\cite{zhao2023verifyandedit}

Annotations

\begin{itemize}
    \item \textbf{Chain-of-Thought (CoT) Prompting}
    \begin{itemize}
        \item \textcolor{red}{Chain-of-Thought (CoT) prompting improves trust and model performance on complex reasoning tasks by generating interpretable reasoning chains, but still suffers from factuality concerns in knowledge-intensive tasks}.
        \item \textcolor{red}{improving the CoT quality could be beneficial in enhancing both interpretability and end-task performance}.
        \item \textcolor{red}{a better set of CoT prompts could provide better grounding and logically consistent thought processes, thus leading to more accurate predictions}.
        \item The commonly proposed methods to improve the factuality of CoT reasoning process can be grouped into two categories: prompt engineering and result calibration.
        \item \textcolor{red}{the lack of supporting facts during the generation process of CoT could largely undermine the validity of the final answer}.
        \item both self-ask and least-to-most prompting still rely on repetitively retrieving internal knowledge learned by the LLM instead of connecting to external knowledge. Thus, their ability to improve factuality is limited.
        \item by feeding in prompts in the format of “question, rationale, answer,” the LLM learns to reason for a few steps before answer generation.
        \item \textcolor{red}{it is of urgent concern to better control the generation and increase the factual correctness of predictions}.
    \end{itemize}

    \item \textbf{Verify-and-Edit (VE) Framework}
    \begin{itemize}
        \item \textcolor{red}{propose the Verify-and-Edit framework for CoT prompting, which seeks to increase prediction factuality by post-editing reasoning chains according to external knowledge}.
        \item Verify-and-Edit (VE) framework to post-edit the reasoning chains for more factually aligned predictions.
        \item \textcolor{red}{we could separate the Verify-and-Edit (VE) framework into 3 different stages: finding uncertain predictions, editing their rationales by searching for supporting facts, and using the edited rationales to generate final answers}.
        \item Deciding when to edit.
        \item How can we identify when a model is unsure of its prediction?
        \item The self-consistency method (Wang et al., 2022) provides a solution. In sampling diverse reasoning paths and answers, self-consistency is found to be highly correlated with accuracy, suggesting that it could provide an uncertainty estimate and confer abilities for the model to “know when it doesn’t know.”
        \item \textcolor{red}{To make the thought process more factually correct, we search for supporting facts in external knowledge sources}.
        \item First, to mimic a human’s query when searching for validating facts, a natural question is generated to verify the rationale.
        \item By generating a relevant question instead of directly querying with the generated rationale, we eliminate potential noise brought by incorrect fact generation.
        \item As the retrieved contexts from a retrieval system could be longer than desired, we use a pre-trained LM to rank and select the top-k sentences most similar to the verifying question query.
        \item with the post-edited CoT, new answers are generated by prompting the LLM.
        \item The Verify-and-Edit framework with open-domain retrieval is able to generate a high accuracy improvement, ranging from 3.4% to 5.9%.
    \end{itemize}

    \item \textbf{Result Calibration and External Knowledge Integration}
    \begin{itemize}
        \item \textcolor{red}{When editing, we first generate a question to verify this detail}.
        \item \textcolor{red}{to answer this query, we introduce external knowledge through open-domain retrieval systems}.
        \item The rationales are edited by providing the retrieved facts in the prompts as memory refreshments.
        \item Result calibration functions on the output of the LLMs.
        \item Wang et al. (2022) propose a self-consistency decoding method, which samples a diverse set of reasoning paths and then selects the most consistent answer by marginalizing out the sampled reasoning paths.
        \item Selection-Inference (SI) (Creswell et al., 2022) framework is another state-of-the-art method that exploits LLMs as general processing modules.
        \item Another comparable line of work has been exploring retrieval-augmented language model pretraining (REALM) (Guu et al., 2020), which first retrieves documents from an external knowledge source and then utilizes retrieved documents to process question-answering tasks.
        \item \textcolor{red}{humans select the reasoning chains produced by Verify-and-Edit as more factually consistent 53\% of the time, compared to 17\% for the CoT-SC baseline}.

    \end{itemize}
    
    \item \textbf{Reasoning Enhancement}
    \begin{itemize}
        \item Reasoning.
        \item To obtain more relevant and logical rationales, we again utilize a natural and generative approach, as reasoning abilities are believed to be already built into LLMs.
        \item we use the verifying questions (as logic) and retrieved facts (as information) to generate informed answers.
    \end{itemize}
    
\end{itemize}

\hfill

\subsubsection{Prioritizing Safeguarding Over Autonomy: Risks of LLM Agents for Science}\cite{tang2024prioritizing}

Annotations


\begin{itemize}
    \item Scientific LLM agents also introduce novel vulnerabilities that demand careful consideration for safety.
    \item This position paper fills this gap by conducting a thorough examination of vulnerabilities in LLM-based agents within scientific domains, shedding light on potential risks associated with their misuse and emphasizing the need for safety measures.
    \item Propose a triadic framework involving human regulation, agent alignment, and an understanding of environmental feedback (agent regulation) to mitigate these identified risks.
    \item A comprehensive risk definition and analysis framework tailored to the scientific context is lacking.
    \item Scientific agents as autonomous systems that have scientific domain capabilities, such as accessing specific biological databases and performing chemical experiments.
    \item Scientific agents can automatically plan and take necessary actions to accomplish the objective.
    \item (1) User Intent, i.e., whether the risk originates from malicious intents or is an unintended consequence of legitimate task objectives.
    \item (2) Scientific Domain, where the agent generates or facilitates risks, encompassing chemical, biological, radiological, physical, and informational risks, as well as those associated with emerging technologies.
    \item (3) Environmental Impact, including the natural environment, human health, and socioeconomic environment affected by such agents.
    \item Informational risks involve the misuse or misinterpretation of data, leading to erroneous conclusions or the unintentional dissemination of sensitive information.
    \item Risks also include the potential leakage of high-stakes information such as private patient data and copyrighted content that are used to train scientific AI agents.
    \item Autonomous agents typically encompass five fundamental modules: LLMs, planning, action, external tools, and memory and knowledge.
    \item Factual Errors.
    \item Vulnerable to Jailbreak Attacks.
    \item Reasoning Capability Deficiencies.
    \item Lack of Up-to-Date Knowledge.
    \item Lack of Awareness of Risks in Long-term Planning.
    \item Deficient Oversight in Tool Usage.
    \item Unreliable Research Sources.
    \item Agents might utilize or train on outdated or unreliable scientific information, leading to the dissemination of incorrect or harmful knowledge.
    \item From LLM Safety to Agent Safety.
    \item Risks encompass issues such as offensiveness, unfairness, illegal activities, and ethical concerns.
    \item Solutions like the self-evaluating and rewinding “RAIN” offer training-free alignment alternatives.
    \item SciGuard has offered a specialized agent for risk control and a benchmark for safety evaluation, where various tools not only assist in executing synthesis instructions but also incorporate long-term memory to enhance safety.
    \item Limitations and Challenges.
    \item (1) Lack of safety constraints on action space and tool usage of agents.
    \item (2) Lack of specialized models for risk control.
    \item (3) Lack of domain-specific expert knowledge.
    \item (4) Ineffective evaluations on the safety of scientific agents.
    \item It has become increasingly evident that the community must prioritize risk control over autonomous capabilities.
    \item We must balance autonomy with security and employ comprehensive strategies to ensure the safe deployment and use of scientific agents.
    \item The emphasis should shift from output safety to behavioral safety, which signifies a comprehensive approach that evaluates not only the accuracy of the agent’s output but also the actions and decisions the agent takes.
    \item Agent Alignment and Safety Evaluation.
    \item Instructions that may pose scientific risks should be included in the human preference datasets, and responses that deal with these threats appropriately should be preferred.
    \item Towards Agent-level Alignment: Different from LLM alignment, agent alignment may focus on the symbolic control of autonomous agents.
    \item Developers must maintain detailed logs of their development activities, algorithms used, and decision-making processes. These records should be accessible for audits and reviews, ensuring accountability and facilitating continuous improvement.
    \item Simulated Environment for Result Anticipation: Scientific agents can significantly benefit from training and operating within simulated environments designed specifically to mimic real-world conditions and outcomes.
    \item Critic Models: Beyond standard safety checks, “critic” models can play a crucial role. These models serve as additional AI layers that assess and refine the outputs of the primary AI system.
    \item Tuning Agents with Action Data: Unlike the setup for LLM Alignment where the aim is to train the LLM, or a direct imposition of an operational procedure on an agent, using annotated data that reflect the potential risks of certain actions can enhance agents’ anticipation of harmful consequences.
\end{itemize}


\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/tang2024-1.png}
    \caption{Vulnerabilities of scientific agents in an autonomous pipeline, Tang \textit{et al.} \cite{tang2024prioritizing}}
    \label{fig:tang2024-1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/tang2024-2.png}
    \caption{Survey of related work in safeguarding LLMs and agents, among which scientific agents are specifically stated, Tang \textit{et al.} \cite{tang2024prioritizing}}
    \label{fig:tang2024-2}
\end{figure}


\hfill

\subsubsection{Control Risk for Potential Misuse of Artificial
Intelligence in Science}\cite{he2023control}

Annotations

\begin{itemize}
    \item \textbf{AI Misuse in Science}
    \begin{itemize}
        \item \textcolor{red}{In this study, we aim to raise awareness of the dangers of AI misuse in science, and call for responsible AI development and use in this domain.}
        \item \textcolor{red}{We propose a system called SciGuard to control misuse risks for AI models in science.}
        \item With the growing prevalence of AI applications in the field of science, worries regarding their potential misapplication are escalating.
        \item \textcolor{red}{Even with good intentions, due to the lack of understanding of these models, scientific AI models might unintentionally cause harm even during regular operation.}
        \item The risks associated with misusing AI models in scientific applications may be even more significant in other general AI domains.
    \end{itemize}
    
    \item \textbf{SciGuard System}
    \begin{itemize}
        \item \textcolor{red}{We propose building safeguarded scientific AI systems, and present SciGuard, as a proof of concept that can mitigate the risks associated with misuse. Furthermore, we build SciMT-Safety, a red-teaming dataset to assess the safety risks of scientific AI systems.}
        \item SciGuard is a system that acts as a mediator between users and scientific AI models, providing a controlled environment where the potential for misuse is minimized.
        \item SciGuard intercepts user queries and model outputs and processes them based on a set of predefined ethical and safety standards, which can be customized for different domains and scenarios.
        \item SciGuard: A System for Controlling the Risks of Misuse for AI Models in Science.
        \item Serve as the middleware, preventing direct access between the user and certain scientific models, thereby making risk control feasible.
        \item \textcolor{red}{Value alignment refers to the ability of the system to infer and respect the underlying intentions and values of the users and the stakeholders and to distinguish between benign and potentially harmful queries and outputs.}
        \item Users can describe their tasks utilizing either natural language or a specified structured format and thereafter receive customized responses from SciGuard.
        \item Enhanced context guides the LLMs in formulating plans, culminating in the execution of a series of actions, such as the utilization of particular scientific models.
    \end{itemize}
    
    \item \textbf{Inaccuracy}
    \begin{itemize}
        \item Inaccuracy.
        \item \textcolor{red}{If AI generates incorrect pattern recognition when analyzing data, it could lead researchers to propose inaccurate hypotheses or draw erroneous conclusions.}
    \end{itemize}
    
    \item \textbf{Unexpected Effects}
    \begin{itemize}
        \item Unexpected effects.
        \item \textcolor{red}{In drug design, AI models might fail to identify the potential side effects of certain compounds.}
    \end{itemize}
    
    \item \textbf{Intellectual Property}
    \begin{itemize}
        \item Intellectual property.
        \item \textcolor{red}{The training of scientific AI models frequently necessitates the utilization of extensive datasets, often derived from patented sources and scholarly articles.}
    \end{itemize}
    
    \item \textbf{Privacy}
    \begin{itemize}
        \item Privacy.
        \item In fields such as medical research or genomics, datasets often contain highly personal information that, if not handled with the utmost care, could lead to breaches of confidentiality and privacy.
    \end{itemize}
    
    \item \textbf{Bias and Discrimination}
    \begin{itemize}
        \item Bias and discrimination.
    \end{itemize}
    
    \item \textbf{General AI vs. AI for Science}
    \begin{itemize}
        \item \textcolor{red}{The risks associated with general AI can often be more immediate and identifiable, but the risks of AI for science may have different ethical and social consequences depending on the context, goal, and application of their use.}
        \item LLMs can be used to design, synthesize, modify, or identify malicious molecules or their uses by generating or interpreting natural language descriptions, instructions, or queries that contain or imply such information or knowledge.
    \end{itemize}
    
    \item \textbf{SciGuard Architecture}
    \begin{itemize}
        \item The architecture of SciGuard consists of four main components: memory, tools, actions, and planning, which are designed to help the agent accurately identify and assess risks in a scientific context.
        \item The architecture of SciGuard, as shown in Figure 10, consists of four main components: memory, tools, actions, and planning.
        \item Memory: The memory component of SciGuard is divided into two segments: short-term and long-term memory.
        \item Short-term memory allows the system to adhere to specific regulations and prevent malicious or harmful outcomes.
        \item Long-term memory ensures that the system has access to comprehensive and up-to-date information, which is critical for accurately assessing task requests and user intent and for detecting and avoiding unexpected effects, misinformation, inaccuracy, or privacy breaches.
        \item Tools: The tools component is equipped with various models and agents that enable SciGuard to accomplish a wide range of scientific tasks.
        \item The scientific agents can perform complex and autonomous tasks that involve multiple steps, such as hypothesis generation, data analysis, or experiment planning.
        \item Actions and Planning: The actions and planning components collectively manage the system’s responses to different tasks and orchestrate its operations, ensuring strategic execution and alignment with stored guidelines and principles.
        \item Enhance SciGuard’s ability to assess risks related to complex requests through Chain of Thought.
    \end{itemize}
    
    \item \textbf{SciMT-Safety and Evaluation}
    \begin{itemize}
        \item SciMT-Safety is specifically designed to benchmark the risks associated with the misuse of AI systems in scientific contexts.
        \item We build a red-team agent with handcrafted few-shot examples to generate a list of risky queries. Then, we manually refined the tasks or queries to enable the target systems to produce more harmful content.
        \item Along with risky queries, we adopt similar schemes to establish a SciMT-Benign query set.
        \item \textcolor{red}{The objective of SciMT-Benign is to evaluate whether the agent can effectively counter the red-teaming while avoiding excessive refusal to respond, thereby preserving its helpfulness.}
        \item For scalable and effective evaluation of different AI systems, we use GPT-4 as a judge to evaluate the task responses in line with current practices.
        \item The average harmlessness score of SciGuard is 4.86, which significantly surpasses the 4.21 score of GPT-4, the underlying LLM used in SciGuard.
        \item Improvement may stem from the fact that large language models (LLMs) are exposed to more descriptive information, aiding in better decision-making.
    \end{itemize}
    
    \item \textbf{Limitations and Challenges}
    \begin{itemize}
        \item \textcolor{red}{SciGuard has several limitations and challenges, which need to be addressed and overcome in future work. One of them is that SciGuard relies on the user’s requests to judge the safety and ethics of the requests or outputs, which may not always be reliable or truthful.}
    \end{itemize}
\end{itemize}


\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/sciguard-1.png}
    \caption{SciGuard framework to control the risks of misuse of scientific models, He \textit{et al.} \cite{he2023control}}
    \label{fig:sciguard-1}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=1\linewidth]{figures/sciguard-2.png}
    \caption{SciGuard architecture with four components: memory, tools, actions, and planning; He \textit{et al.} \cite{he2023control}}
    \label{fig:sciguard-1}
\end{figure}


\subsubsection{RAIN: RAIN: Your Language Models Can Align Themselves without Finetuning}\cite{DBLP:conf/iclr/LiWZ0024}

Annotations

\begin{itemize}
    \item \textbf{LLM Alignment}
    \begin{itemize}
        \item \textcolor{red}{Aligning frozen LLMs without requiring alignment data is more appealing.}
        \item \textcolor{red}{The problem of LLM alignment becomes more challenging when we require the model to be aligned by itself without external supervision, a.k.a. self-alignment.}
        \item \textcolor{red}{By integrating evaluation and the rewind mechanism, frozen LLMs can directly generate responses that are consistent with human values.}
        \item \textcolor{red}{Alignment with reinforcement learning.}
        \item \textcolor{red}{Alignment without reinforcement learning.}
    \end{itemize}

    \item \textbf{Rewindable Auto-regressive INference (RAIN)}
    \begin{itemize}
        \item \textcolor{red}{We introduce a novel inference method, Rewindable Auto-regressive INference (RAIN), that allows pre-trained LLMs to evaluate their own generation and use the evaluation results to guide rewind and generation for AI safety.}
        \item \textcolor{red}{RAIN improves the harmlessness rate of LLaMA 30B from 82\% of vanilla inference to 97\%.}
        \item \textcolor{red}{On the TruthfulQA dataset, RAIN improves the truthfulness of the well-aligned LLaMA-2-chat 13B model by 5\%.}
        \item \textcolor{red}{Our inference method—Rewindable Auto-regressive INference (RAIN)—mirrors human behavioral patterns: contemplating, weighing, and reflecting on the consequences before speaking.}
        \item \textcolor{red}{Rewindable Auto-regressive INference (RAIN).}
        \item \textcolor{red}{RAIN conducts searches on the tree consisting of token sets and dynamically reduces the weight of harmful token sets, with backward rewind and forward generation steps until the output content is self-evaluated as harmless.}
        \item \textcolor{red}{The inner loop alternates between forward and backward steps to update token set attributes, allowing tokens to be rewound and modified.}
        \item \textcolor{red}{The outer loop, utilizing updated attributes, adjusts token set probabilities and sequentially determines the next token set, with confirmed tokens becoming immutable.}
        \item RAIN appears identical to vanilla auto-regressive inference if one only looks at the outer loop.
        \item \textcolor{red}{In the inner loop, we initiate a search commencing from the previously determined tokens, treated as the root node.}
        \item \textcolor{red}{To improve the efficiency of the search, the search direction is determined using the previously recorded value v and visit count n.}
        \item The search direction should consider both exploitation and exploration, that is, favoring token sets with higher value and fewer explorations.
    \end{itemize}

    \item \textbf{Evaluation and Performance}
    \begin{itemize}
        \item \textcolor{red}{We discover that by integrating self-evaluation and rewind mechanisms, unaligned LLMs can directly produce responses consistent with human preferences via self-boosting.}
        \item \textcolor{red}{Employing a prompt, enabling the model to conduct self-evaluations of its production.}
        \item \textcolor{red}{To counter potential biases from the model’s preference for Label A or B, we swap the label-content mapping (A/B and harmless/harmful), utilizing the average score for evaluation.}
        \item \textcolor{red}{The value v of the token set Ya:b in the context of Y1:b should be the average score s of token sequences that have Y1:b as a prefix.}
        \item \textcolor{red}{For small-scale models, RAIN slightly reduces helpfulness, but this gap reduces with large-scale models, which means for adequately large models, RAIN does not hurt performance on other objectives.}
        \item A naïve trade-off between computation and performance is multiple rounds of random search, generating text via vanilla autoregressive sampling and choosing the language model’s preferred text as the final output.
        \item Even with 500 trials, for the 7B model, sample-evaluation scarcely enhances the model’s safety; whereas, with the 30B model, RAIN demonstrates significantly better performance.
        \item GPT-4 evaluations align closely with human assessments.
    \end{itemize}

    \item \textbf{Techniques and Strategies}
    \begin{itemize}
        \item \textcolor{red}{Lookahead and backtracking.}
        \item \textcolor{red}{Adversarial attack on LLMs.}
    \end{itemize}
\end{itemize}


\hfill

\subsection{Guardrail Tooling \& Frameworks}

\begin{itemize}
    \item FACTOOL: Factuality Detection in Generative AI - A Tool Augmented Framework for Multi-Task and Multi-Domain Scenarios\cite{chern2023factool}
    \item Fact or Fiction: Verifying Scientific Claims\cite{wadden2020fact}
    \item Jailbroken: How Does LLM Safety Training Fail?\cite{weiJailbrokenHowDoes}
    \item “Aligning with whom? Large language models have gender and racial biases in subjective NLP tasks”\cite{sun2023aligning}
    \item LLama Guard
    \item Nvidia NeMo - \href{https://github.com/NVIDIA/NeMo-Guardrails/blob/develop/docs/user_guides/colang-language-syntax-guide.md}{$https://github.com/NVIDIA/NeMo-Guardrails/blob/develop/docs/user_guides/colang-language-syntax-guide.md$}
    \item Guardrails AI - \href{https://github.com/guardrails-ai/guardrails}{$https://github.com/guardrails-ai/guardrails$}
    \item TruLens - \href{https://github.com/truera/trulens}{$https://github.com/truera/trulens$}
    \item Guidance AI - \href{https://github.com/guidance-ai/guidance/}{$https://github.com/guidance-ai/guidance/$}
    \item LMQL - \href{https://github.com/eth-sri/lmql}{$https://github.com/eth-sri/lmql$}
    \item AIF360 - \href{https://github.com/Trusted-AI/AIF360?tab=readme-ov-file}{$https://github.com/Trusted-AI/AIF360?tab=readme-ov-file$}
    \item FairLearn - \href{https://fairlearn.org/}{$https://fairlearn.org/$}
    \item Detoxify - \href{https://github.com/unitaryai/detoxify}{$https://github.com/unitaryai/detoxify$}
    \item ToolEmu: Identifying the Risks of LM Agents with an LM-Emulated Sandbox - \href{https://github.com/ryoungj/ToolEmu?tab=readme-ov-file}{$https://github.com/ryoungj/ToolEmu?tab=readme-ov-file$}
\end{itemize}

\subsection{To Read}

\begin{itemize}
    \item \href{https://arxiv.org/pdf/2309.02705}{Certifying LLM Safety against Adversarial Prompting}
    \item \href{https://arxiv.org/abs/2403.13031}{RigorLLM: Resilient Guardrails for Large Language Models against Undesired Content}
    \item \href{https://arxiv.org/abs/2308.07308}{LLM Self Defense: By Self Examination, LLMs Know They Are Being Tricked}
\end{itemize}


\subsection{Scratchpad}

\subsubsection{Thoughts 1}

\begin{table}[H]
\centering
\caption{Key Challenges and Safeguards Categorized by Guardrail Types}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Key Challenges and Safeguards} & \textbf{White-Box Guardrail} & \textbf{Gray-Box Guardrail} & \textbf{Black-Box Guardrail} \\ \hline
\textbf{Preventing Hallucinations}     & Formal Verification          & LoRA (Low-Rank Adaptation)  & Rule-Based Filtering, Retrieval-Augmented Generation \\ \hline
\textbf{Ensuring Data Fairness}        & Internal Bias Mitigation     & External Bias Mitigation    & Content Moderation, Rule-Based Filtering \\ \hline
\textbf{Protecting Privacy}            & -                            & Differential Privacy        & Rule-Based Filtering, Content Moderation \\ \hline
\textbf{Enhancing Robustness}          & Adversarial Training         & LoRA (Low-Rank Adaptation)  & Red-Teaming \& Testing \\ \hline
\textbf{Content Control}               & -                            & -                           & Content Moderation, Rule-Based Filtering \\ \hline
\textbf{Legal Compliance}              & Formal Verification          & Differential Privacy        & Rule-Based Filtering, Content Moderation \\ \hline
\textbf{Managing Unusual Data}         & Formal Verification          & LoRA (Low-Rank Adaptation)  & Rule-Based Filtering, Retrieval-Augmented Generation \\ \hline
\textbf{Uncertainty Quantification}    & Formal Verification          & LoRA (Low-Rank Adaptation)  & Rule-Based Filtering \\ \hline
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{|p{0.3\textwidth}|p{0.3\textwidth}|p{0.3\textwidth}|}
\hline
\textbf{White-box Guardrails} & \textbf{Black-box Guardrails} & \textbf{Gray-box Guardrails} \\
\hline
Formal verification & Post-processing filters & Hybrid verification approaches \\
\hline
Adversarial training & Output sampling and reranking & Uncertainty-aware output generation \\
\hline
Architecture modifications & External fact-checking systems & Prompt engineering for accuracy \\
\hline
Constrained decoding & API-based content moderation & Selective fine-tuning \\
\hline
Embedding safety checks & Input sanitization & Interpretability-enhanced models \\
\hline
\end{tabular}
\caption{Guardrail Implementation Strategies for LLMs in Scientific Applications}
\label{tab:guardrails}
\end{table}


\subsubsection{notes}

Put this in paragraph somewhere in key-aspect section:
[Conflicting Research Results, fill=red!30, align=left]

==> chapter-3-old.tex <==
\section{Dimensions for Guardrails for Science}

In the previous section, we identified various gaps in applying general LLM guardrails to the scientific domain, such as the lack of domain-specific adaptation, insufficient temporal relevance, and challenges in handling multidisciplinary data. Here we propose a set of tailored areas that address and encompass those properties within specific scientific needs. 

These dimensions are categorized under four main areas: \textit{Trustworthiness}, \textit{Ethics \& Bias}, \textit{Safety}, and \textit{Legal}. Each category is further subdivided into critical areas for improvement, offering a roadmap for applying LLM guardrails more effectively within scientific contexts.

The dimensions are represented in a structured framework, illustrated in Figure \ref{forest:llm-guardrails-science-tree}, and categorized by the level of adaptation required. We use a color-coding scheme -- blue, orange, red, and uncolored -- to indicate the extent of modification needed for existing LLM guardrails to be applied to scientific research. Blue boxes signify areas where minimal adaptation is necessary, orange boxes denote dimensions that require some refinement, red boxes represent areas where significant development is required, and uncolored boxes represent a categorization that indicates areas already addressed by LLMs across multiple domains, rather than specific, well-defined guardrails.

Below, we expand each category, highlighting key dimensions and explaining their importance in scientific research.

\begin{figure}[!h]
\centering
\begin{forest}
for tree={
    grow=east,
    draw,
    rounded corners,
    edge={-stealth},
    l sep=2cm, % Adjust horizontal spacing
    s sep=0.8cm, % Adjust vertical spacing
    parent anchor=east,
    child anchor=west,
    calign=center,
    calign primary angle=0,
    calign secondary angle=0,
    fit=band,
    scale=.7,
    anchor=base west,
}
[Key Aspects of LLM Guardrails in Scientific Domains,
    [Trustworthiness,
        [Explainability,
            [Verification, fill=blue!30]
            [Uncertainty Identification, fill=blue!30]
            [Attribution, fill=orange!30]
        ]
        [Factuality, name=factuality,
            [Consistency, fill=blue!30]
            [Hallucination Identification, fill=orange!30]
            [Knowledge Contextualization, fill=red!30]
            [Time Sensitivity, fill=red!30]
        ]
    ]
    [Ethics \& Bias,
        [Fairness, fill=blue!30]
        [Societal Impact, fill=orange!30]
    ]
    [Safety,
        [Robustness,
            [Jailbreak Prevention, fill=blue!30]
            [Out of Distribution Checks, fill=blue!30]
        ]
        [Harmfulness Detection,
            [Toxicity, fill=blue!30]
            [Profanity, fill=blue!30]
            [Maliciousness, fill=blue!30]
        ]
    ]
    [Legal, name=legal,
        [Privacy, fill=blue!30]
        [Compliance, fill=blue!30]
        [IP \& Copyright, fill=red!30]
    ]
]
\end{forest}
\caption{Key Aspects of LLM Guardrails in Scientific Domains}
\label{forest:llm-guardrails-science-tree}
\end{figure}

\subsection{Blue Boxes}

The blue boxes represent the dimensions of LLM guardrails that can be adapted for scientific use with minimal modification. These are established best practices that can transition smoothly into the scientific context, requiring only slight adjustments. The goal here is to leverage these existing guardrails to enhance LLMs for the specific needs of scientific research, ensuring their outputs are dependable and contextually appropriate. The following dimensions outline the key areas where LLM guardrails must be implemented to ensure they are suitable for scientific research. These dimensions aim to enhance the reliability, safety, and ethical compliance of LLM outputs

\begin{itemize}
    \item \textbf{Verification:} 
    Ensuring that LLM outputs can be verified against known, established sources.
    
    \item \textbf{Uncertainty Identification:} 
    Mechanisms for identifying uncertainty in LLM outputs.
    
    \item \textbf{Consistency:} 
    Maintaining consistency in information, particularly concerning scientific data.
    
    \item \textbf{Fairness:} 
    Addressing fairness concerns to prevent biased or prejudiced outputs.
    
    \item \textbf{Robustness:} 
    Strengthening LLMs against potential failures, including jailbreak prevention and out-of-distribution checks.
    
    \item \textbf{Harmfulness Detection:} 
    Detecting harmful outputs related to toxicity, profanity, and maliciousness.
    
    \item \textbf{Privacy:} 
    Ensuring LLMs comply with privacy laws and safeguard personal information.

    \item \textbf{Compliance:} 
    Ensuring that LLMs adhere to legal, ethical, and institutional guidelines. 
\end{itemize}


\subsubsection{Compliance}

The \textbf{Compliance} dimension ensures that the identification of similar research work and relevant grants adhere to legal, ethical, and institutional guidelines, while also promoting trustworthiness in scientific research. This functionality is critical for optimizing resource allocation, avoiding research duplication, and fostering collaboration. This also focuses on developing sophisticated tools that can automatically search and compare existing literature, grant opportunities, and ongoing research projects, thereby aiding researchers in navigating the vast and ever-expanding body of scientific knowledge. For instance, an LLM could analyze a researcher’s proposal and automatically suggest related studies or previous work in the same area, helping to ensure that the new research builds on existing knowledge rather than inadvertently replicating it. No guardrail dimensions exist yet that address this problem. While there has been some work \cite{zhu2023novel} on matching grants in a specific domain, there has yet to be proper discipline on the implementation in a wider scientific domain.

Similarly, it also ensures that the works follow publication guidelines and scientific values. Identifying related grants is particularly valuable for researchers seeking funding opportunities that align with their projects. By scanning grant databases and matching them with the researcher's area of study, LLMs can suggest relevant funding opportunities, streamlining the grant application process and increasing the chances of securing support. This functionality saves time and opens up potential collaborations by identifying research groups working on similar problems.

The development of these capabilities would require LLMs to perform comprehensive searches and analyses, cross-referencing multiple sources of academic literature and funding databases. Advanced natural language processing (NLP) techniques would be necessary to accurately parse and understand the nuanced details of research proposals and grant descriptions, ensuring that the recommendations \cite{wu24survey} made are highly relevant and useful to the researchers.

Incorporating these search and comparison tools into LLMs would empower researchers to make more informed decisions, enhance the efficiency of the research process, and foster a more collaborative scientific community. These tools represent a significant step toward integrating AI more deeply into the research lifecycle, supporting the broader goals of innovation and knowledge advancement in the scientific community. \cite{floridi2022unified}

\subsection{Orange boxes}

The orange boxes represent existing dimensions but require significant refinement to meet the unique demands of scientific integrity, accountability, and precision. These dimensions are crucial in ensuring that LLMs provide accurate outputs, uphold ethical standards, and promote contextual understanding within scientific disciplines.

\begin{itemize}
    \item \textbf{Attribution:} 
    Ensuring proper credit to original sources to maintain academic integrity.  
    
    \item \textbf{Hallucination Identification:} 
    The ability to recognize when LLMs provide inaccurate or fabricated information.
    
    \item \textbf{Societal Impact:} 
    Considering the broader societal effects of LLM-generated outputs.
    
\end{itemize}


\subsubsection{Attribution}
Proper attribution is essential in scientific research to acknowledge original sources, avoid plagiarism, and maintain academic integrity. LLMs may inadvertently generate content that closely mirrors existing literature without appropriate citations, raising concerns about intellectual dishonesty and transparency of LLM-generated content. To address this, LLMs must be incorporated with mechanisms for accurate attribution, such as generating citations in the correct academic formats, implementing source-tracking capabilities, and integrating plagiarism detection algorithms. \cite{gao2022rarr} \cite{bohnet2022attributed}

Challenges include the complexity of source materials, knowledge cutoffs \cite{zhu2024llm} leading to outdated citations, and variability in citation styles across disciplines. Strategies to improve attribution involve integrating LLMs with citation databases like PubMed or CrossRef, employing retrieval-augmented generation techniques \cite{lewis2020retrieval} to access the latest publications, and standardizing citation practices within the models. By prioritizing accurate attribution, LLMs can enhance the trustworthiness of their outputs, uphold ethical standards, and facilitate verification of information, thereby fostering a more transparent and reliable scientific community.

\subsection{Red boxes} 

The red boxes represent dimensions where current LLM guardrails are either underdeveloped to meet scientific standards, or non-existent in the general literature. These areas are crucial for the future development of LLMs tailored to scientific research.

\subsubsection{Time Sensitivity}

LLMs are trained on static datasets with a specific knowledge cutoff date and lack mechanisms for real-time knowledge updates \cite{zhu2024llm} \cite{mousavi2024dyknowdynamically}. This limitation presents several critical issues with relying on LLMs for scientific applications:

\begin{itemize}
    \item \textbf{Rapid Obsolescence}: In evolving scientific fields like epidemiology, biotechnology, or climate science, research findings and policy changes occur frequently and information can become obsolete within months or weeks. LLMs, however, are "frozen" at their last point of training, meaning they cannot incorporate or reflect the most recent advancements unless explicitly retrained. This rapid obsolescence is especially problematic in domains where timely, accurate information is essential for decision-making, such as public health, finance, or crisis management.
    \item \textbf{False Confidence}: One of the challenges with LLMs is their ability to present outdated information with high confidence, making it difficult for users to discern whether the information provided is still accurate or relevant. LLMs do not have built-in mechanisms to flag their knowledge is outdated unless they are explicitly prompted to consider the possibility. For example, a scientist using an LLM for advice on the latest vaccine technologies may receive responses that seem authoritative but reflect research that is no longer cutting-edge. The model's high confidence in outdated data can lead to misguided conclusions or recommendations, as the LLM is unable to signal that newer research might have changed the consensus.
    \item \textbf{Lack of Real-time Updates}: Unlike human experts who continuously update their knowledge through ongoing research, conferences, and real-time data, LLMs remain static after their training phase. This limitation becomes problematic in situations where real-time updates are critical. For instance, financial markets, geopolitical conflicts, or pandemics evolve in real-time, requiring access to the most current data to make informed decisions. An LLM cannot respond to breaking news or incorporate real-time information about stock market crashes, viral outbreaks, or sudden regulatory changes, making it less reliable for applications requiring up-to-the-minute insights. This static nature limits its utility in environments that demand agility and current knowledge. 
    \item \textbf{Potential for Misinformation}: In a worst-case scenario, relying on outdated information from an LLM could lead to significant consequences, including the spread of misinformation or misguided actions. In fields like public health, for instance, outdated data could result in misallocation of critical resources or ineffective strategies. Imagine a scenario where public health officials used an LLM to guide vaccination strategies based on old data that does not reflect the emergence of new viral variants. This could result in ineffective public health measures, such as promoting vaccines that are less effective against new strains, leading to increased infection rates, unnecessary strain on healthcare systems, and a failure to protect vulnerable populations. Misinformation stemming from outdated models could exacerbate crises instead of mitigating them.

\end{itemize}

Therefore, as scientific knowledge is dynamic and constantly evolving, LLMs must provide information that is not only accurate but also temporally relevant. The challenge is that many LLMs are trained on datasets that may become outdated \cite{zhu2024llm} \cite{mousavi2024dyknowdynamically}, leading to the generation of content that no longer reflects the current state of scientific understanding. To address this, models need to be equipped with mechanisms to verify the temporal validity of information by cross-referencing against real-time data sources. This could involve integrating LLMs with updated knowledge bases or using retrieval-augmented generation (RAG) \cite{lewis2020retrieval} techniques to pull in current information as part of the response generation process. 

\subsubsection{Knowledge Contextualization}

Similar to time sensitivity, LLM responses must adapt their responses to the specific context in which information is applied. In scientific research, the same data can produce varying conclusions depending on the region, field of study, or unique circumstances of the user’s inquiry. \textbf{Knowledge contextualization} ensures that LLMs take these variations into account, allowing for more nuanced, tailored responses. This means recognizing disciplinary differences, adjusting recommendations based on the user’s level of expertise, and considering geographical or environmental factors that may influence how a particular piece of knowledge should be applied. By understanding the context, LLMs can offer outputs that are not only factually correct but also pragmatically relevant to the specific research or situation at hand.

For example, in agricultural research, a general recommendation on farming best practices may be valid for a temperate region but completely unsuitable for arid climates. A lack of contextualization could result in crop damage or environmental harm. LLMs need the ability to adapt information dynamically to reflect these unique local conditions, which often requires an understanding of diverse disciplines, localized expertise, and complex interdependencies within the context of a specific inquiry. Below are key challenges that emerge when LLMs fail to properly contextualize knowledge:

\begin{itemize}

\item \textbf{Overgeneralization:}
LLMs often provide generalized responses that fail to account for local variations or specific situational needs. This can lead to recommendations that are ineffective or even harmful when applied in contexts with unique environmental, demographic, or infrastructural factors. Overgeneralization risks poor decision-making and unintended negative consequences, particularly in domains like agriculture and healthcare, where local conditions are critical for successful outcomes.

\item \textbf{Failure to Integrate Multidisciplinary Knowledge:}
LLMs often struggle to synthesize information from multiple disciplines, providing narrow, discipline-specific responses. This can lead to incomplete or unbalanced recommendations, particularly in complex fields like sustainable farming, where solutions require integrating knowledge from climatology, ecology, economics, and soil science. The lack of multidisciplinary integration may result in decisions that optimize one aspect while neglecting others, leading to suboptimal or harmful outcomes, even if the query to LLM might seem benign. One potential mitigation strategy could be to adapt LLMs to use tools that incorporate these disciplines. \cite{lu2024chameleon}

\item \textbf{Lack of Adaptive Reasoning:}
LLMs often lack the ability to adjust their responses to the specific context of a problem, such as local economic, environmental, or social factors. Adaptive reasoning \cite{chentoward} \cite{DBLP:conf/emnlp/AggarwalY23} requires weighing multiple, sometimes conflicting variables, which LLMs struggle to do effectively. Without this ability, they may offer one-size-fits-all recommendations that overlook critical nuances, leading to poor decision-making and undesirable outcomes in areas like public policy, healthcare, or disaster management.
\end{itemize}

Additionally, it is common to encounter studies with differing conclusions involving the synthesis of conflicting data and perspectives. Current LLMs may struggle to handle these conflicts effectively \cite{xu2024knowledge}, leading to oversimplified or biased outputs. LLMs need to be able to identify and appropriately manage these conflicts, rather than presenting conflicting results as equally valid without distinction. Therefore, it is necessary to develop frameworks that allow LLMs to recognize, reconcile, and accurately represent conflicting findings in scientific literature. This would involve integrating advanced reasoning algorithms like chain-of-thoughts \cite{wei2022chain}, chain-of-verification \cite{dhuliawala2023chain}, verify-and-edit \cite{zhao2023verifyandedit} that can weigh evidence, evaluate the credibility of sources, and present balanced conclusions. Furthermore, solutions could involve developing models that can prioritize information based on the consensus within the scientific community or highlight the divergence in findings to guide users in making informed decisions. Conflict resolution mechanisms within LLMs could be employed to manage these situations effectively \cite{liu-etal-2024-untangle} \cite{chern2023factool}.

\subsubsection{IP \& Copyright}

Intellectual property (IP) and copyright play a fundamental role in scientific research, where the originality and ownership of ideas, data, and innovations are crucial \cite{sobel2017artificial}. This dimension focuses on developing mechanisms within LLMs that can accurately identify, track, and manage intellectual property and copyrighted content, ensuring that the outputs generated respect the proprietary rights of researchers, institutions, and other stakeholders. By integrating these capabilities, LLMs can uphold legal and ethical standards, maintaining the integrity of the scientific process while protecting the rights of individuals and organizations.

As LLMs generate content, it is crucial to recognize and label portions of text that may be novel, patentable, or otherwise protected under intellectual property laws \cite{sobel2017artificial}. This capability is essential not only for protecting IP rights but also for guiding researchers and organizations in managing and utilizing these outputs. For instance, if an LLM generates an innovative idea or a unique piece of content, the system should be able to flag this as potentially patentable, alerting users to the need for further steps to secure IP protection \cite{chesterman2024good}.

Moreover, ensuring that attribution of sources is a vital component of IP and copyright management. LLMs should be equipped with citation and attribution mechanisms to accurately acknowledge the origins of data, ideas, or prior work referenced in generated content. This preserves academic integrity and mitigates legal risks related to IP infringement or unauthorized use of proprietary information. By doing so, the system can identify instances where the output may require licensing or other legal compliance before it can be used commercially \cite{abdikhakimov2023unraveling}.

This proposed categorization of LLM guardrails addresses the complex challenges of using LLMs in scientific applications that emphasize trust, ethical responsibility, safety, and legal compliance. We focused primarily on dimensions highlighted by the red boxes, which represent areas where current LLM guardrails are insufficient for the scientific domain. In the following section, we outline implementation strategies for enhancing these guardrails, categorized as white-box, black-box, and gray-box approaches to meet the unique demands of the scientific domain.

